The Performance of Photometric Reverberation Mapping at High Redshift and the Reliability of Damped Random Walk Models

Accurate methods for reverberation mapping using photometry are highly sought after since they are inherently less resource intensive than spectroscopic techniques. However, the effectiveness of photometric reverberation mapping for estimating black hole masses is sparsely investigated at redshifts higher than $z\approx0.04$. Furthermore, photometric methods frequently assume a Damped Random Walk (DRW) model, which may not be universally applicable. We perform photometric reverberation mapping using the Javelin photometric DRW model for the QSO SDSSJ144645.44+625304.0 at z=0.351 and estimate the H$\beta$ lag of $65^{+6}_{-1}$ days and black-hole mass of $10^{8.22^{+0.13}_{-0.15}}M_{\odot}$. An analysis of the reliability of photometric reverberation mapping, conducted using many thousands of simulated CARMA process light-curves, shows that we can recover the input lag to within 6 per cent on average given our target's observed signal-to-noise of > 20 and an average cadence of 14 days (even when DRW is not applicable). Furthermore, we use our suite of simulated light curves to deconvolve aliases and artefacts from our QSO's posterior probability distribution, increasing the signal-to-noise on the lag by a factor of $\sim2.2$. We exceed the signal-to-noise of the Sloan Digital Sky Survey Reverberation Mapping Project (SDSS-RM) campaign with a quarter of the observing time per object, resulting in a $\sim200$ per cent increase in SNR efficiency over SDSS-RM.

==> fit_table.tex <==
\begin{table}
\centering
\begin{tabular}{cccc}
\toprule
{} &                        $\hat{K}$ &                   $\hat{\alpha}$ &                  $\log[\hat{\epsilon}]$ \\
\midrule
Clean2+ExtCorr+\\Target10 &  $1.541_{-0.002}^{+0.001}$ &  $0.494_{-0.001}^{+0.001}$ &  $-0.542_{-0.005}^{+0.005}$ \\
\midrule
Clean2+ExtCorr          &  $1.539_{-0.002}^{+0.001}$ &  $0.480_{-0.001}^{+0.001}$ &  $-0.623_{-0.005}^{+0.004}$ \\
\midrule
Clean2+ExtCorr\\(Bentz+13) & $1.559\pm0.024$ &  $0.549_{-0.027}^{+0.028}$ & $\sim-1.016_{-0.187}^{+0.169}$\\
\bottomrule
\end{tabular}
\caption{Lag fit parameters for datasets with and without \TargetTen. 
The fit results from \citet{Bentz2013LowLuminosity} are included but the scatter has been approximately converted to the power law model using $\epsilon \approx 10^{\sigma} -1$  for comparison.}
\label{tab:RM:fit_parameters}
\end{table}


==> numbers.tex <==
\newcommand{\TargetTenFullName}{\texttt{SDSSJ144645.44+625304.0}\xspace}
\newcommand{\TargetTen}{Target-10\xspace}
\newcommand{\TargetTenCadence}{14 days\xspace}
\newcommand{\TargetTenMinSNR}{\ensuremath{>20}\xspace}
\newcommand{\TargetTenRedshift}{0.351}
\newcommand{\SplineGradientTolerance}{$0.05$ mag\xspace}
\newcommand{\SDSSMagnitudeAggreement}{$0.05$ mag\xspace}
\newcommand{\AutocorrelationTimeTolerance}{1 per cent\xspace}
\newcommand{\AutocorrelationTimeMultiple}{50\xspace} % how many autocorrelation times to run the chain for
\newcommand{\JavelinNWalkers}{200\xspace}
\newcommand{\NumberOfSimulatedLightCurves}{50\,000\xspace}
\newcommand{\TargetTenReferenceSpectrumRaDec}{\ensuremath{\alpha_{J2000} = 14^{h}46^{m}37^{s},  \delta_{J2000} = +62\degree 57\amin 36\asec}}
\newcommand{\TargetTenLagPeakLow}{63 days\xspace}
\newcommand{\TargetTenLagPeakHigh}{72 days\xspace}

\newcommand{\TargetTenUninformedLag}{\ensuremath{73^{+4}_{-13}} days\xspace}
\newcommand{\TargetTenInformedLag}{\ensuremath{65^{+6}_{-1}} days\xspace}
\newcommand{\TargetTenInformedSNR}{\ensuremath{18.6}\xspace}
\newcommand{\TargetTenLagUncertaintyWidth}{7 days\xspace}
\newcommand{\SNRIncrease}{\ensuremath{\sim 2.2}\xspace}
\newcommand{\TargetTenUninformedMass}{\ensuremath{10^{8.27_{-0.15}^{+0.13}} \mathrm{M_{\odot}}}\xspace}
\newcommand{\TargetTenInformedMass}{\ensuremath{10^{8.22^{+0.13}_{-0.15}}\mathrm{M_{\odot}}}\xspace}
\newcommand{\ffactor}{\ensuremath{\langle f \rangle = 4.3 \pm 1.1}\xspace}
\newcommand{\AverageLagRecoveryErrorLessThan}{6 per cent\xspace}
\newcommand{\ReliableLagsBelow}{170 days\xspace}
\newcommand{\IterativeReweightingTolerance}{0.001 mag\xspace}
\newcommand{\NumberOfBlackHoleMasses}{100\xspace}
\newcommand{\EfficiencyPercentIncrease}{218 per cent\xspace}
\newcommand{\RoughEfficiencyPercentIncrease}{$\sim$ 200 per cent\xspace}
\newcommand{\TargetTenBaseline}{330 days}

==> target_table.tex <==
\begin{table*}
\centering
\begin{tabular}{ccccccccccccc}
\toprule
 & RA & Dec & & $i_{AB}$ & $\lambda L_{5100}$ & $t_{H\beta}(1+z)$ & \multicolumn{2}{c}{visibility} & \multicolumn{2}{c}{epochs} & \multicolumn{2}{c}{observed baseline}\\
SDSS ID &          /\degree &        /\degree &       z &   /mag & /$\log[\mathrm{erg s^{-1}}]$ & /days & /days & /$t_{H\beta}(1+z)$ & \halpha & \iband & /days & /$t_{H\beta}(1+z)$\\
\midrule
J082905.01+571541.6 &   127.2708 &   57.2615 &   0.350 &   17.9 &     44.24 &       61.4 &             250 &          4.1 & 0 & 0 & 0 & 0\\
J153601.07+162838.4 &   234.0044 &   16.4773 &   0.382 &   17.9 &     44.35 &       72.2 &             301 &          4.2 & 16 & 14 & 208 & 2.9\\
J112600.00+304005.3 &   171.5000 &   30.6681 &   0.361 &   17.9 &     44.41 &       76.1 &             231 &          3.0 & 0 & 0 & 0 & 0\\
J122519.30+372053.6 &   186.3304 &   37.3482 &   0.388 &   17.9 &     44.45 &       81.9 &             249 &          3.0 & 11 & 11 & 180 & 2.2\\
J154246.51+194626.1 &   235.6938 &   19.7739 &   0.398 &   17.9 &     44.46 &       83.1 &             305 &          3.7 & 0 & 0 & 0 & 0\\
J150243.09+111557.3 &   225.6795 &   11.2659 &   0.390 &   17.5 &     44.56 &       93.4 &             278 &          3.0 & 0 & 0 & 0 & 0\\
J153057.45+304322.0 &   232.7393 &   30.7228 &   0.378 &   17.6 &     44.57 &       93.5 &             314 &          3.4 & 17 & 19 & 189 & 2.0\\
J164224.30+444509.8 &   250.6012 &   44.7527 &   0.368 &   17.8 &     44.58 &       94.5 &             334 &          3.5  & 16 & 15 & 179 & 1.9\\
J153729.23+272250.7  &  234.3717  &  27.3807  &  0.388  &  17.9  &     44.57 &       95.0 &             312 &          3.3 & 0 & 0 & 0 & 0\\
\textbf{J144645.44+625304.0} &   \textbf{221.6893} &   \textbf{62.8844} &   \textbf{0.351} &   \textbf{17.8} &     \textbf{44.45} &       \textbf{91.7} &             \textbf{337} &          \textbf{3.7} & \textbf{31} & \textbf{30} & \textbf{329} & \textbf{3.6}\\
\bottomrule
\end{tabular}
\caption{Our pre-observation targets selected based on their luminosity, redshift and visibility. 
$t_{H\beta}(1+z)$ is expected observed-frame lag derived from the \citet{Bentz2013LowLuminosity} $t_{\mathrm{rest}}-L_{5100}$ relation, where $L_{5100}$ is estimated from the SDSS spectrum. 
We quote the length of time each target is visible and the baseline of the observations in units of days and expected observed-frame lag.}
\label{tab:RM:targets}
\end{table*}
% Target names = 1, 2, 3, 4, 5, 13, 14, 16, 19, 10

